Confidence-aware Reward Optimization for Fine-tuning Text-to-Image Models

Fine-tuning text-to-image models with reward functions trained on human feedback data has proven effective for aligning model behavior with human intent. However, excessive optimization with such reward models, which serve as mere proxy objectives, can compromise the performance of fine-tuned models, a phenomenon known as reward overoptimization. To investigate this issue in depth, we introduce the Text-Image Alignment Assessment (TIA2) benchmark, which comprises a diverse collection of text prompts, images, and human annotations. Our evaluation of several state-of-the-art reward models on this benchmark reveals their frequent misalignment with human assessment. We empirically demonstrate that overoptimization occurs notably when a poorly aligned reward model is used as the fine-tuning objective. To address this, we propose TextNorm, a simple method that enhances alignment based on a measure of reward model confidence estimated across a set of semantically contrastive text prompts. We demonstrate that incorporating the confidence-calibrated rewards in fine-tuning effectively reduces overoptimization, resulting in twice as many wins in human evaluation for text-image alignment compared against the baseline reward models.

==> tables/benchmark_category_allocation.tex <==
\footnotesize
\tcbox[colback=white,boxrule=1pt,arc=3mm]{
\begin{tblr}[c]{@{}X@{}}
Given input is the caption for generated image. Allocate input prompt with all applicable categories. Do not allocate categories that can't be derived from input prompt.\\
Below is the total categories that can be allocated.\\
format: (Category:Explanation)\\
Creative: This category involves imaginative and unconventional representations of objects.\\
Spatial: This category related to the arrangement and relationship of objects in space.\\
Text: In this category, Specific text must be mentioned.
Style: This category is focused on creating images in specific artistic styles or imitating the aesthetics of certain characters or scenes.\\
Counting: This category involves images with a specific number of items. It's about depicting a precise quantity of objects within an image, offering a straightforward visual representation of numbers.\\
Colors: This category focuses on depicting objects with specific, sometimes unconventional colors. \\
Composition: This category involves combining different objects or entities in a single image. The focus is on the arrangement and relationship between these elements. It's about how various elements coexist within a single frame.\\
Location: This category is about placing objects or creatures in specific locations or settings. It emphasizes the context or environment surrounding the subject of the image.\\\\
Categories:[Creative,Spatial,Text,Style,Counting,Colors,Composition,Location]\\\\

output: [Category allocation reason],[Corresponding categories]\\
\textcolor{blue}{[few\_shot\_examples]}
\end{tblr}}

==> tables/benchmark_evaluation_instruction.tex <==
\begin{tabularx}{0.95\textwidth}{|X|}
    \hline
    \textbf{Instruction} \\ \hline
    For each pair of images, you will be asked two questions to assess\\
    (1) which of the two is more consistent with the input prompt\\
    (2) which of the two is of better quality\\\\

    Note: In case both images are inconsistent with the prompt and yet one is clearly closer to the prompt than the other, please select the one closer. If both are roughly equally wrong, please select neither, i.e., label “3”.\\
    \hline  
\end{tabularx}


==> tables/benchmark_stats.tex <==
\begin{tabularx}{0.65\textwidth}{lcc*{2}{Y}}
    \toprule
    \small
    \multirow{2}{*}{Category} & \multirow{2}{14mm}{No. of prompts} & \multirow{2}{14mm}{No. of images} & \multicolumn{2}{c}{Human labels (\%)} \\
    \cmidrule(lr){4-5}
    & & & Good & Bad \\
    \midrule
    Comprehensive & 100 & 5,000 & 47.22 & 52.78 \\
    Counting & 150 & 7,500 & 43.27 & 56.73 \\
    Composition & 300 & 15,000 & 38.97 & 61.03 \\
    \midrule
    Total & 550 & 27,500 & 41.64 & 58.36 \\
    \bottomrule
\end{tabularx}

